Semantically Tied Paired Cycle Consistency for Zero-Shot Sketch-based Image Retrieval

Zero-shot sketch-based image retrieval (SBIR) is an emerging task in computer vision, allowing to retrieve natural images relevant to sketch queries that might not been seen in the training phase. Existing works either require aligned sketch-image pairs or inefficient memory fusion layer for mapping the visual information to a semantic space. In this work, we propose a semantically aligned paired cycle-consistent generative (SEM-PCYC) model for zero-shot SBIR, where each branch maps the visual information to a common semantic space via an adversarial training. Each of these branches maintains a cycle consistency that only requires supervision at category levels, and avoids the need of highly-priced aligned sketch-image pairs. A classification criteria on the generators' outputs ensures the visual to semantic space mapping to be discriminating. Furthermore, we propose to combine textual and hierarchical side information via a feature selection auto-encoder that selects discriminating side information within a same end-to-end model. Our results demonstrate a significant boost in zero-shot SBIR performance over the state-of-the-art on the challenging Sketchy and TU-Berlin datasets.

==> tex/qual_results_sketchy.tex <==
\begin{figure*}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/bear} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/2_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/3_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/6_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/8_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/9_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/5/20_1} \\
 & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/geyser} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/6/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/wheelchair} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/3_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/7_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/8_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/12/20_1} \\
 & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/lobster} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/13/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/spoon} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/5_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/16_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/23/20_1} \\
 & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/trumpet} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/3_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/5_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/6_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/17_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/29/20_0} \\
 & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/squirrel} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/41/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/rhinoceros} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/6_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/11_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/16_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/48/20_0} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/hamburger} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/4_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/54/20_1} \\ 
 & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/bell} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/55/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/racket} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/2_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/4_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/9_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/17_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/65/20_1} \\ 
 & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/teapot} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/16_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/66/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/cannon} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/68/20_0} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/motorcycle} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/3_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/16_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/70/20_1} \\ 
 & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/mushroom} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/7_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/71/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/jack_o_lantern} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/5_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/7_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{sketchy/106/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark \\
\end{tabular}
}
\end{center}
\caption{Top-20 zero-shot SBIR results obtained by our SEM-PCYC model on the Sketchy dataset are shown here according to the Euclidean distances, where the green ticks denote the correctly retrieved candidates, whereas the red crosses indicate the wrong retrievals. (best viewed in color)}
\label{fig:qual_results_sketchy}
\end{figure*}

==> tex/qual_results_tuberlin.tex <==
\begin{figure*}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/snail} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/7_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/11_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/2/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/truck} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/5_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/4/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/umbrella} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/7/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/hedgehog} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/9/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/snake} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/10/20_0} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/table_lamp} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/14/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/knife} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/15/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/couch} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/3_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/8_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/9_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/16_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/17_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/17/20_1} \\ 
 & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/duck} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/2_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/5_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/11_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/17_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/21/20_1} \\ 
 & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/walkie_talkie} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/9_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/17_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/27/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/bookshelf} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/1_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/6_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/7_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/32/20_0} \\ 
 & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark \\
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/eyeglasses} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/46/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/foot} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/5_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/6_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/9_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/10_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/12_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/15_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/16_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/17_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/19_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/89/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/calculator} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/90/20_1} \\ 
 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/snowman} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/3_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/4_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/11_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/13_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/14_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/18_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/95/20_1} \\ 
 & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\ 
\includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/rollerblades} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/1_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/2_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/3_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/4_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/5_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/6_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/7_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/8_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/9_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/10_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/11_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/12_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/13_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/14_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/15_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/16_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/17_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/18_0} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/19_1} & \includegraphics[width=1.5cm, height=1.5cm]{tu-berlin/130/20_0} \\ 
 & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark \\ 
\end{tabular}
}\end{center}
\caption{Top-20 zero-shot SBIR results obtained by our SEM-PCYC model on the TU-Berlin dataset are shown here according to the Euclidean distances, where the green ticks denote the correctly retrieved candidates, whereas the red crosses indicate the wrong retrievals. (best viewed in color)}
\label{fig:qual_results_tu-berlin}
\end{figure*}

% \caption{Top-20 zero-shot SBIR results obtained by our SEM-PCYC model are shown here according to the Euclidean distances, where the green ticks denote the correctly retrieved candidates, whereas the red crosses indicate the wrong retrievals. (best viewed in pdf)}
